Investigation of Accuracy and Bias in Face Recognition Trained with Synthetic Data

Synthetic data has emerged as a promising alternative for training face recognition (FR) models, offering advantages in scalability, privacy compliance, and potential for bias mitigation. However, critical questions remain on whether both high accuracy and fairness can be achieved with synthetic data. In this work, we evaluate the impact of synthetic data on bias and performance of FR systems. We generate balanced face dataset, FairFaceGen, using two state of the art text-to-image generators, Flux.1-dev and Stable Diffusion v3.5 (SD35), and combine them with several identity augmentation methods, including Arc2Face and four IP-Adapters. By maintaining equal identity count across synthetic and real datasets, we ensure fair comparisons when evaluating FR performance on standard (LFW, AgeDB-30, etc.) and challenging IJB-B/C benchmarks and FR bias on Racial Faces in-the-Wild (RFW) dataset. Our results demonstrate that although synthetic data still lags behind the real datasets in the generalization on IJB-B/C, demographically balanced synthetic datasets, especially those generated with SD35, show potential for bias mitigation. We also observe that the number and quality of intra-class augmentations significantly affect FR accuracy and fairness. These findings provide practical guidelines for constructing fairer FR systems using synthetic data.

==> sections/diagram.tex <==

\tikzstyle{process} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black, fill=gray!10]
\tikzstyle{arrow} = [thick,->,>=stealth]

\begin{tikzpicture}[node distance=1.5cm]

% Nodes
\node (prompt) [process] {Prompt-Based};
\node (flux) [process, left=3cm of prompt] {Flux};
\node (sd35) [process, right=3cm of prompt] {SD35};

\node (identities) [process, below=of prompt] {Different Identities (Balanced: Race, Age, Gender)};
\node (augment) [process, below=of identities] {Augmentation};
\node (arc2face) [process, left=3cm of augment] {Arc2Face};
\node (ipadapters) [process, right=3cm of augment] {IP-Adapters};

\node (output) [process, below=of augment] {Synthetic Dataset};

% Arrows
\draw [arrow] (flux) -- (prompt);
\draw [arrow] (sd35) -- (prompt);
\draw [arrow] (prompt) -- (identities);
\draw [arrow] (identities) -- (augment);
\draw [arrow] (arc2face) -- (augment);
\draw [arrow] (ipadapters) -- (augment);
\draw [arrow] (augment) -- (output);

\end{tikzpicture}

